Hubble Constant Measurement from Three Large-Separation Quasars Strongly Lensed by Galaxy Clusters

Tension between cosmic microwave background-based and distance ladder-based determinations of the Hubble constant ${\rm H}_{\rm 0}$ motivates pursuit of independent methods that are not subject to the same systematic effects. A promising alternative, proposed by Refsdal in 1964, relies on the inverse scaling of ${\rm H}_{\rm 0}$ with the delay between the arrival times of at least two images of a strongly-lensed variable source such as a quasar. To date, Refsdal's method has mostly been applied to quasars lensed by individual galaxies rather than by galaxy clusters. Using the three quasars strongly lensed by galaxy clusters (SDSS J1004+4112, SDSS J1029+2623, and SDSS J2222+2745) that have both multiband Hubble Space Telescope data and published time delay measurements, we derive ${\rm H}_{\rm 0}$, accounting for the systematic and statistical sources of uncertainty. While a single time delay measurement does not yield a well-constrained ${\rm H}_{\rm 0}$ value, analyzing the systems together tightens the constraint. Combining the six time delays measured in the three cluster-lensed quasars gives ${\rm H}_{\rm 0}$ = 74.1 $\pm$ 8.0 km s$^{-1}$ Mpc$^{-1}$. To reach 1$\%$ uncertainty in ${\rm H}_{\rm 0}$, we estimate that a sample size of order of 620 time delay measurements of similar quality as those from SDSS J1004+4112, SDSS J1029+2623, and SDSS J2222+2745 would be needed. Improving the lens modeling uncertainties by a factor of two and a half may reduce the needed sample size to 100 time delays, potentially reachable in the next decade.

==> longtable.tex <==
\begin{center}
\begin{longtable}{lllll}
\hline
System & ID & R.A. [J2000] & Decl. [J2000] & \textit{z} \\
\hline
\SDSSfiveim & & & & \\
& QSO-A & 151.1450074 & 41.2109193 & 1.734 \\
& QSO-B & 151.1454888 & 41.2119003 & 1.734 \\
& QSO-C & 151.1409266 & 41.2096668 & 1.734 \\
& QSO-D & 151.1419060 & 41.2136092 & 1.734 \\
& QSO-E & 151.1423413 & 41.2122017 & 1.734 \\
& 2.1 & 151.1418821 & 41.2102917 & 2.74 \\
& 2.2 & 151.1468800 & 41.2153908 & 2.74 \\ 
& 21.1 & 151.1417325 & 41.2103272 & 2.74 \\
& 21.2 & 151.1470383 & 41.2153011 & 2.74 \\
& 21.3 & 151.1419526 & 41.2116044 & 2.74 \\
& 22.1 & 151.1416225 & 41.2103033 & 2.74 \\
& 22.2 & 151.1471250 & 41.2152436 & 2.74 \\
& 3.1 & 151.1414121 & 41.2099250 & 3.288 \\
& 3.2 & 151.1476847 & 41.2152121 & 3.288 \\
& 31.1 & 151.1413250 & 41.2099825 & 3.288 \\
& 31.2 & 151.1477393 & 41.2151976 & 3.288 \\
& 32.1 & 151.1412104 & 41.2100544 & 3.288 \\
& 32.2 & 151.1478065 & 41.2151979 & 3.288 \\
& 33.1 & 151.1411279 & 41.2101547 & 3.288 \\
& 33.2 & 151.1478809 & 41.2151884 & 3.288 \\
& 33.3 & 151.1418864 & 41.2116948 & 3.288 \\
& 4.1 & 151.1439081 & 41.2165866 & 3.332 \\ 
& 4.2 & 151.1382517 & 41.2153846 & 3.332 \\  
& 4.3 & 151.1379048 & 41.2149959 & 3.332 \\  
& 4.4 & 151.1434099 & 41.2103752 & 3.332 \\  
& 41.1 & 151.1441118 & 41.2165193 & 3.332 \\  
& 41.2 & 151.1383309 & 41.2153297 & 3.332 \\  
& 41.3 & 151.1378932 & 41.2148820 & 3.332 \\  
& 41.4 & 151.1434562 & 41.2102573 & 3.332 \\  
& 42.1 & 151.1444522 & 41.2163884 & 3.332 \\  
& 42.2 & 151.1383940 & 41.2153469 & 3.332 \\  
& 42.3 & 151.1378407 & 41.2148091 & 3.332 \\  
& 42.4 & 151.1434818 & 41.2101761 & 3.332 \\  
& 43.1 & 151.1445319 & 41.2162919 & 3.332 \\  
& 43.2 & 151.1384506 & 41.2154232 & 3.332 \\  
& 43.3 & 151.1376594 & 41.2145747 & 3.332 \\  
& 43.4 & 151.1435603 & 41.2101349 & 3.332 \\   
& 43.5 & 151.1424833 & 41.2118271 & 3.332 \\ 
% & & & & \\
\SDSSthreeim & & & & \\
& QSO-A & 157.3081009 & 26.38830445 & 2.1992 \\ 
& QSO-B & 157.3093619 & 26.39446237 & 2.1992 \\  
& QSO-C & 157.3095755 & 26.3939894 & 2.1992 \\  
& 1.1 & 157.2980611 & 26.3907404 & - \\
& 1.2 & 157.2978817 & 26.3924467 & - \\
& 1.3 & 157.3008758 & 26.3974054 & - \\
& 2.1 & 157.2981743 & 26.3915325 & 2.1812 \\
& 2.3 & 157.3014749 & 26.3977063 & 2.1812 \\
& 3.1 & 157.2990642 & 26.3923892 & 3.0275 \\
& 3.2 & 157.3074114 & 26.3913469 & 3.0275 \\
& 3.3 & 157.3041512 & 26.3982630 & 3.0275 \\
& 3.4 & 157.3015481 & 26.3880193 & 3.0275 \\  
& 3.5 & 157.3017377 & 26.3879213 & 3.0275 \\  
& 3.6 & 157.3018385 & 26.3878900 & 3.0275 \\  
& 3.7 & 157.3032208 & 26.3919632 & 3.0275 \\
& 4.1 & 157.2992278 & 26.3925219 & 3.0278 \\
& 4.2 & 157.3076382 & 26.3913247 & 3.0278 \\
& 4.3 & 157.3043869 & 26.3981437 & 3.0278 \\
& 4.4 & 157.3023985 & 26.3877048 & 3.0278 \\
& 4.5 & 157.3035100 & 26.3920169 & 3.0278 \\
& 5.1 & 157.3019777 & 26.3946563 & 1.0232 \\ 
& 5.3 & 157.3008781 & 26.3917377 & 1.0232 \\ 
& 7.1 & 157.3075794 & 26.3951262 & 5.0622 \\
& 7.2 & 157.3064130 & 26.3960500 & 5.0622 \\ 
& 7.3 & 157.3014210 & 26.3936610 & 5.0622 \\ 
& 7.4 & 157.3012420 & 26.3938020 & 5.0622 \\ 
% & & & & \\
%\SDSSsixim & & & & \\
%& QSO-A & 335.537707 & 27.760543 & 2.805 \\  
%& QSO-B & 335.53669 & 27.761119 & 2.805 \\     
%& QSO-C & 335.53296 & 27.760505 & 2.805 \\     
%& QSO-D & 335.536205 & 27.758901 & 2.805 \\     
%& QSO-E & 335.536007 & 27.758248 & 2.805 \\     
%& QSO-F & 335.535874 & 27.759723 & 2.805 \\  
%& 11.1 & 335.53687 & 27.761148 & 2.805 \\   
%& 11.2 & 335.53751 & 27.760801 & 2.805 \\   
%& 11.3 & 335.532945 & 27.760637 & 2.805 \\   
%& 13.1 & 335.53704 & 27.760914 & 2.805 \\ 
%& 13.2 & 335.53734 & 27.760733 & 2.805 \\
%& 2.4 & 335.53505 & 27.757058 & 2.2963 \\   
%& 2.5 & 335.53484 & 27.757115 & 2.2963 \\  
%& 4.1 & 335.53388 & 27.757979 & 4.562 \\   
%& 4.2 & 335.53482 & 27.75763 & 4.562 \\      
%& 4.3 & 335.53841 & 27.758236 & 4.562 \\   
%& 41.1 & 335.53398 & 27.757948 & 4.562 \\   
%& 41.2 & 335.53473 & 27.757663 & 4.562 \\   
%& 6.1 & 335.53551 & 27.761518 & - \\    
%& 6.2 & 335.53842 & 27.760385 & - \\    
%& 6.3 & 335.53362 & 27.760879 & - \\ 
%& 5.1 & 335.53353 & 27.755175 & - \\    
%& 5.2 & 335.53409 & 27.754942 & - \\    
%& 5.3 & 335.53454 & 27.754882 & - \\ 
\caption{Positions and spectroscopic redshifts of the multiply-imaged background sources used as constraints in the strong lens models for \SDSSfiveim\ and \SDSSthreeim.  See Table 1 from \cite{Sharon2017} for the lensing constraints for \SDSSsixim.}  
\label{table:constraints}
\end{longtable}
\end{center}
